Linear Bandits with Memory: from Rotting to Rising

Nonstationary phenomena, such as satiation effects in recommendations, have mostly been modeled using bandits with finitely many arms. However, the richer action space provided by linear bandits is often preferred in practice. In this work, we introduce a novel nonstationary linear bandit model, where current rewards are influenced by the learner's past actions in a fixed-size window. Our model, which recovers stationary linear bandits as a special case, leverages two parameters: the window size $m \ge 0$, and an exponent $\gamma$ that captures the rotting ($\gamma < 0)$ or rising ($\gamma > 0$) nature of the phenomenon. When both $m$ and $\gamma$ are known, we propose and analyze a variant of OFUL which minimizes regret against cycling policies. By choosing the cycle length so as to trade-off approximation and estimation errors, we then prove a bound of order $\sqrt{d}\,(m+1)^{\frac{1}{2}+\max\{\gamma,0\}}\,T^{3/4}$ (ignoring log factors) on the regret against the optimal sequence of actions, where $T$ is the horizon and $d$ is the dimension of the linear action space. Through a bandit model selection approach, our results are extended to the case where $m$ and $\gamma$ are unknown. Finally, we complement our theoretical results with experiments against natural baselines.

==> list_of_related.tex <==
Cited in the initial draft:

% Learning to optimize under non-stationarity
% Adaptive exploration in linear contextual bandits
% Randomized exploration for non-stationary stochastic linear bandits
% Algorithms for non-stationary generalized linear bandits
% Weighted linear bandits for non-stationary environments
% A simple approach for non-stationary linear bandits

Unrelated but to be cited:

% A New Algorithm for Non-stationary Contextual Bandits: Efficient, Optimal, and Parameter-free
% -> regret bounds against finitely many policies in terms of changepoints and TV

% Learning Contextual Bandits in a Non-stationary Environment
% -> LinUCB with changepoints, regret bounds in terms of changepoints

% Low-Rank Bandit Methods for High-Dimensional Dynamic Pricing
% -> Application of nonstationary linear bandits to dynamic pricing

% Unifying Clustered and Non-stationary Bandits
% -> non-stationarity in linear bandit with time-varying arm set

% Weighted Gaussian Process Bandits for Non-stationary Environments
% -> Linear bandits in a RKHS

% A Technical Note on Non-Stationary Parametric Bandits: Existing Mistakes and Preliminary Solutions
% -> This note identifies technical flaws in some of the papers cited above

